Weakly Labeling the Antarctic: The Penguin Colony Case

Antarctic penguins are important ecological indicators -- especially in the face of climate change. In this work, we present a deep learning based model for semantic segmentation of Ad\'elie penguin colonies in high-resolution satellite imagery. To train our segmentation models, we take advantage of the Penguin Colony Dataset: a unique dataset with 2044 georeferenced cropped images from 193 Ad\'elie penguin colonies in Antarctica. In the face of a scarcity of pixel-level annotation masks, we propose a weakly-supervised framework to effectively learn a segmentation model from weak labels. We use a classification network to filter out data unsuitable for the segmentation network. This segmentation network is trained with a specific loss function, based on the average activation, to effectively learn from the data with the weakly-annotated labels. Our experiments show that adding weakly-annotated training examples significantly improves segmentation performance, increasing the mean Intersection-over-Union from 42.3 to 60.0% on the Penguin Colony Dataset.

==> temp.tex <==

\begin{table}[]
\centering
\caption{\textbf{A-Net classification results on the weakly-annotated set of the Penguin Colony Dataset.} The label ``Pos''. denotes the patches containing penguin guano areas and ``Neg.'' denotes patches containing only backgrounds}
\label{tab:A-Net2}
\setlength{\tabcolsep}{15pt}
\begin{tabular}{llll}
                                                 &                            & \multicolumn{2}{c}{\textit{``Label''}}                              \\ \cline{3-4} 
                                                 & \multicolumn{1}{l|}{}      & \multicolumn{1}{l|}{Pos.} & \multicolumn{1}{l|}{Neg.} \\ \cline{2-4} 
\multicolumn{1}{l|}{\multirow{2}{*}{\textit{Pred.}}} & \multicolumn{1}{l|}{Pos.}  & \multicolumn{1}{l|}{9597}  & \multicolumn{1}{l|}{2070}   \\ \cline{2-4} 
\multicolumn{1}{l|}{}                            & \multicolumn{1}{l|}{Neg.} & \multicolumn{1}{l|}{19446}   & \multicolumn{1}{l|}{69471}  \\ \cline{2-4} 
\end{tabular}
\end{table}
